Comparative Analysis of Information Theoretic and Statistical Methods for Line Parameter Estimation

Recent studies indicate that the noise characteristics of phasor measurement units (PMUs) can be more accurately described by non-Gaussian distributions. Consequently, estimation techniques based on Gaussian noise assumptions may produce poor results with PMU data. This paper considers the PMU based line parameter estimation (LPE) problem, and investigates the performance of four state-of-the-art techniques in solving this problem in presence of non-Gaussian measurement noise. The rigorous comparative analysis highlights the merits and demerits of each technique w.r.t. the LPE problem, and identifies conditions under which they are expected to give good results.

==> bibilography1.tex <==
@article{shen2015minimum,
  title={Minimum total error entropy method for parameter estimation},
  author={Shen, Pengcheng and Li, Chunguang},
  journal={IEEE Trans. Signal Process.},
  volume={63},
  number={15},
  pages={4079--4090},
  year={2015},
  publisher={IEEE}
}

@article{wang2017maximum,
  title={Maximum total correntropy adaptive filtering against heavy-tailed noises},
  author={Wang, Fei and He, Yicong and Wang, Shiyuan and Chen, Badong},
  journal={Signal Process.},
  volume={141},
  pages={84--95},
  year={2017},
  publisher={Elsevier}
}

@article{QIAN2021107903,
title = {Robust constrained maximum total correntropy algorithm},
journal = {Signal Process.},
volume = {181},
pages = {107903},
year = {2021},
issn = {0165-1684},
doi = {https://doi.org/10.1016/j.sigpro.2020.107903},
author = {Guobing Qian and Fuliang He and Shiyuan Wang and H.C. Iu Herbert},
}

@ARTICLE{varghese2022transmission,
  author={Varghese, Antos Cheeramban and Pal, Anamitra and Dasarathy, Gautam},
  journal={IEEE Trans. Power Syst.}, 
  title={Transmission Line Parameter Estimation Under Non-{G}aussian Measurement Noise}, 
  year={2023},
  volume={38},
  number={4},
  pages={3147-3162},
  doi={10.1109/TPWRS.2022.3204232}}

@book{kelley1995iterative,
  title={Iterative methods for linear and nonlinear equations},
  author={Kelley, Carl T},
  year={1995},
  publisher={SIAM}
}

@article{shi2011transmission1,
  title={{Transmission line parameter identification using PMU measurements}},
  author={Shi, Di and Tylavsky, Daniel J and Koellner, Kristian M and Logic, Naim and Wheeler, David E},
  journal={European Trans. Electrical Power},
  volume={21},
  number={4},
  pages={1574--1588},
  year={2011},
  publisher={Wiley Online Library}
}


@article{zimmerman2010matpower,
  title={MATPOWER: Steady-state operations, planning, and analysis tools for power systems research and education},
  author={Zimmerman, Ray Daniel and Murillo-S{\'a}nchez, Carlos Edmundo and Thomas, Robert John},
  journal={IEEE Trans. Power Syst.},
  volume={26},
  number={1},
  pages={12--19},
  year={2010},
  publisher={IEEE}
}

@article{ritzmann_method_2016,
	title = {A {Method} for {Accurate} {Transmission} {Line} {Impedance} {Parameter} {Estimation}},
	volume = {65},
	issn = {1557-9662},
	doi = {10.1109/TIM.2016.2556920},
	abstract = {Real-time estimation of power transmission line impedance parameters has become possible with the availability of synchronized phasor (synchrophasor) measurements of voltage and current. If sufficiently accurate, the estimated parameter values are a powerful tool for improving the performance of a range of power system monitoring, protection, and control applications, including fault location and dynamic thermal line rating. The accuracy of the parameter estimates can be reduced by unknown errors in the synchrophasors that are introduced in the measurement process. In this paper, a method is proposed with the aim of obtaining accurate estimates of potentially variable impedance parameters, in the presence of systematic errors in voltage and current measurements. The method is based on optimization to identify correction constants for the phasors. A case study of a simulated transmission line is presented to demonstrate the effectiveness of the new method, which is better in comparison with a previously proposed method. The results, as well as limits, and the potential extensions of the new method are discussed.},
	number = {10},
	journal = {IEEE Trans. Instrum. Meas.},
	author = {Ritzmann, Deborah and Wright, Paul S. and Holderbaum, William and Potter, Ben},
	month = oct,
	year = {2016},
	keywords = {Accuracy, admittance measurement, Current measurement, Impedance, impedance measurement, Measurement uncertainty, optimization methods, parameter estimation, phasor measurement unit (PMU), Power transmission lines, Systematics, transmission line measurements, Transmission line measurements, Voltage measurement},
	pages = {2204--2213},
	file = {IEEE Xplore Full Text PDF:C\:\\Users\\avarghe6\\Zotero\\storage\\9DQ6DCM8\\Ritzmann et al. - 2016 - A Method for Accurate Transmission Line Impedance .pdf:application/pdf;IEEE Xplore Abstract Record:C\:\\Users\\avarghe6\\Zotero\\storage\\WG9Z4KWJ\\7465793.html:text/html},
}

@article{du2012line1,
  title={On-line estimation of transmission line parameters, temperature and sag using {PMU} measurements},
  author={Du, Yan and Liao, Yuan},
  journal={Electric Power Syst. Research},
  volume={93},
  pages={39--45},
  year={2012},
  publisher={Elsevier}
}

@article{lin2019synchrophasor,
  title={Synchrophasor data analytics: Transmission line parameters online estimation for energy management},
  author={Lin, Junjie and Song, Jie and Lu, Chao},
  journal={IEEE Trans. Eng. Manag.},
  year={2019},
  pages={1-11},
  publisher={IEEE}
}

@article{xue2019linear,
  title={{Linear approximations for the influence of phasor angle difference errors on line parameter calculation}},
  author={Xue, Ancheng and Xu, Feiyang and Martin, Kenneth E and Xu, Jingsong and You, Hongyu and Bi, Tianshu},
  journal={IEEE Trans. Power Syst.},
  volume={34},
  number={5},
  pages={3455--3464},
  year={2019},
  publisher={IEEE}
}



@article{wehenkel2020parameter,
  title={Parameter estimation of three-phase untransposed short transmission lines from synchrophasor measurements},
  author={Wehenkel, Antoine and Mukhopadhyay, Arpan and Le Boudec, Jean-Yves and Paolone, Mario},
  journal={IEEE Trans. Instrum. Meas.},
  volume={69},
  number={9},
  pages={6143--6154},
  year={2020},
  publisher={IEEE}
}


@article{gupta2021compound,
  title={Compound Admittance Matrix Estimation of Three-Phase Untransposed Power Distribution Grids Using Synchrophasor Measurements},
  author={Gupta, Rahul Kumar and Sossan, Fabrizio and Le Boudec, Jean-Yves and Paolone, Mario},
  journal={IEEE Trans. Instrum. Meas.},
  volume={70},
  pages={1--13},
  year={2021},
  publisher={IEEE}
}

@article{ahmad2019statistical,
  title={{Statistical characterization of PMU error for robust WAMS based analytics}},
  author={Ahmad, Tabia and Senroy, Nilanjan},
  journal={IEEE Trans. Power Syst.},
  volume={35},
  number={2},
  pages={920--928},
  year={2019},
  publisher={IEEE}
}


@article{wang2017assessing,
  title={{Assessing Gaussian assumption of PMU measurement error using field data}},
  author={Wang, Shaobu and Zhao, Junbo and Huang, Zhenyu and Diao, Ruisheng},
  journal={IEEE Trans. Power Del.},
  volume={33},
  number={6},
  pages={3233--3236},
  year={2017},
  publisher={IEEE}
}




@inproceedings{mishra2015kalman_1,
  title={Kalman-filter based recursive regression for three-phase line parameter estimation using synchrophasor measurements},
  author={Mishra, Chetan and Centeno, Virgilio A and Pal, Anamitra},
  booktitle={2015 IEEE Power \& Energy Soc. General Meeting},
  pages={1--5},
  year={2015}
}

@article{yu2017patopa_1,
  title={{PaToPa: A data-driven parameter and topology joint estimation framework in distribution grids}},
  author={Yu, Jiafan and Weng, Yang and Rajagopal, Ram},
  journal={IEEE Trans. Power Syst.},
  volume={33},
  number={4},
  pages={4335--4347},
  year={2017},
  publisher={IEEE}
}


@article{gurusinghe2017efficient,
  title={Efficient algorithms for real-time monitoring of transmission line parameters and their performance with practical synchrophasors},
  author={Gurusinghe, Dinesh Rangana and Rajapakse, Athula D},
  journal={IET Generation, Transmission \& Distribution},
  volume={11},
  number={5},
  pages={1134--1143},
  year={2017},
  publisher={IET}
}


@article{milojevic2018utilization_1,
  title={{Utilization of PMU measurements for three-phase line parameter estimation in power systems}},
  author={Milojevi{\'c}, Vladimir and {\v{C}}alija, Srdan and Rietveld, Gert and A{\v{c}}anski, Milo{\v{s}} V and Colangelo, Daniele},
  journal={IEEE Trans. Instrum. Meas.},
  volume={67},
  number={10},
  pages={2453--2462},
  year={2018},
  publisher={IEEE}
}

@INPROCEEDINGS{mansani2018estimation,
  author={Mansani, Prashanth Kumar and Pal, Anamitra and Rhodes, Matthew and Keel, Brian},
  booktitle={2018 IEEE North American Power Symp. (NAPS)}, 
  title={Estimation of Transmission Line Sequence Impedances using Real {PMU} Data}, 
  year={2018},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/NAPS.2018.8600605}}

@INPROCEEDINGS{mishra2015kalman,
  author={Mishra, Chetan and Centeno, Virgilio A. and Pal, Anamitra},
  booktitle={2015 IEEE Power \& Energy Soc. General Meeting}, 
  title={Kalman-filter based recursive regression for three-phase line parameter estimation using synchrophasor measurements}, 
  year={2015},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/PESGM.2015.7285678}}

@INPROCEEDINGS{ding2011transmission,
  author={Ding, Lan and Bi, Tianshu and Zhang, DaoNong},
  booktitle={2011 Int. Conf. Adv. Power Syst. Autom. Protection}, 
  title={{Transmission line parameters identification based on moving-window TLS and PMU data}}, 
  year={2011},
  volume={3},
  number={},
  pages={2187-2191},
  doi={10.1109/APAP.2011.6180790}}

@INPROCEEDINGS{salls2021statistical,
  author={Salls, Demetra and Torres, Jairo Ramírez and Varghese, Antos Cheeramban and Patterson, John and Pal, Anamitra},
  booktitle={2021 IEEE Power \& Energy Soc. General Meeting}, 
  title={Statistical Characterization of Random Errors Present in Synchrophasor Measurements}, 
  year={2021},
  volume={},
  number={},
  pages={01-05},
  doi={10.1109/PESGM46819.2021.9638135}}


@article{chatterjee2018error,
  title={Error reduction of phasor measurement unit data considering practical constraints},
  author={Chatterjee, Paroma and Pal, Anamitra and Thorp, James S and Lopez, Jaime De La Ree and Centeno, Virgilio A},
  journal={IET Generation, Transmission \& Distribution},
  volume={12},
  number={10},
  pages={2332--2339},
  year={2018},
  publisher={IET}
}

@article{asprou2017identification,
  title={Identification and estimation of erroneous transmission line parameters using PMU measurements},
  author={Asprou, Markos and Kyriakides, Elias},
  journal={IEEE Trans. Power Del.},
  volume={32},
  number={6},
  pages={2510--2519},
  year={2017},
  publisher={IEEE}
}


@article{golub1980analysis,
  title={An analysis of the total least squares problem},
  author={Golub, Gene H and Van Loan, Charles F},
  journal={SIAM J. numerical analysis},
  volume={17},
  number={6},
  pages={883--893},
  year={1980},
  publisher={SIAM}
}


@article{markovsky2007overview,
  title={Overview of total least-squares methods},
  author={Markovsky, Ivan and Van Huffel, Sabine},
  journal={Signal Process.},
  volume={87},
  number={10},
  pages={2283--2302},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{kusic2004measurement,
  title={Measurement of transmission line parameters from {SCADA} data},
  author={Kusic, G. L. and Garrison, D. L.},
  booktitle={2004 IEEE Power \& Energy Soc. Power Syst. Conf. Exposition},
  pages={440--445},
  year={2004}
}

@misc{IEEE_IEC2018PMU_Std,
  author={},
  journal={IEC/IEEE 60255-118-1:2018}, 
  title={{IEEE/IEC} International Standard - Measuring relays and protection equipment - Part 118-1: Synchrophasor for power systems - Measurements}, 
  year={2018},
  volume={},
  number={},
  pages={1-78},
  doi={10.1109/IEEESTD.2018.8577045}}

@article{tapia1974newton,
  title={Newton’s method for optimization problems with equality constraints},
  author={Tapia, RA},
  journal={SIAM J. Numerical Analysis},
  volume={11},
  number={5},
  pages={874--886},
  year={1974},
  publisher={SIAM}
}

@inproceedings{gao2012dynamic,
  title={Dynamic state prediction based on auto-regressive {(AR)} model using {PMU} data},
  author={Gao, Fenghua and Thorp, James S and Pal, Anamitra and Gao, Shibin},
  booktitle={2012 IEEE Power \& Energy Conf. Illinois},
  pages={1--5},
  year={2012}
}

@article{albuquerque2021estimation,
  title={Estimation of transmission line parameters by using two least-squares methods},
  author={Albuquerque, Felipe P and Costa, Eduardo C Marques and Liboni, Lu{\'\i}sa HB and Pereira, Ronaldo F Ribeiro and de Oliveira, Maur{\'\i}cio C},
  journal={IET Generation, Transmission \& Distribution},
  volume={15},
  number={3},
  pages={568--575},
  year={2021},
  publisher={Wiley Online Library}
}

@article{goklani2023robust,
  title={A robust method for transmission line sequence parameter estimation using synchronized phasor measurements},
  author={Goklani, Hemantkumar and Gajjar, Gopal and Soman, SA},
  journal={Electric Power Syst. Research},
  volume={223},
  pages={109616},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{dasgupta2013line,
  title={Line parameter estimation using phasor measurements by the total least squares approach},
  author={Dasgupta, Kalyan and Soman, SA},
  booktitle={2013 IEEE Power \& Energy Soc. General Meeting},
  pages={1--5},
  year={2013}
}

@article{castello2022statistical,
  title={Statistical behavior of {PMU} measurement errors: An experimental characterization},
  author={Castello, Paolo and Muscas, Carlo and Pegoraro, Paolo Attilio},
  journal={IEEE Open J. Instrum. Meas.},
  volume={1},
  pages={1--9},
  year={2022},
  publisher={IEEE}
}

@article{varghese2023timesynchronized,
  title={Time-Synchronized Full System State Estimation Considering Practical Implementation Challenges},
  author={Antos Cheeramban Varghese and Hritik Shah and Behrouz Azimian and Anamitra Pal and Evangelos Farantatos},
  journal={J. Modern Power Syst. Clean Energy},
  note={To appear},
  year={2024},
  publisher={IEEE}
}
